One size doesn't fit all: Predicting the Number of Examples for In-Context Learning

In-context learning (ICL) refers to the process of adding a small number of localized examples from a training set of labelled data to an LLM's prompt with an objective to effectively control the generative process seeking to improve the downstream task performance. Existing ICL approaches use an identical number of examples (a pre-configured hyper-parameter) for each data instance. Our work alleviates the limitations of this 'one fits all' approach by dynamically predicting the number of examples for each data instance to be used in few-shot inference with LLMs. In particular, we employ a multi-label classifier, the parameters of which are fitted using a training set, where the label for each instance in this training set indicates if using a specific value of k (number of most similar examples from 0 up to a maximum value) leads to correct k-shot downstream predictions. Our experiments on a number of text classification benchmarks show that AICL substantially outperforms standard ICL by up to 17%.

==> figdefs/diff_frac_kpredictor.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.32\textwidth]{figs/agnews_cropped.pdf}
\includegraphics[width=0.32\textwidth]{figs/toxicity_cropped.pdf}
\includegraphics[width=0.32\textwidth]{figs/sst2_cropped.pdf}
\caption{
Sensitivity of AICL (LLM: OPT-2.7B) to the size of training data used to learn the number of examples on the AGNews, Toxicity and SST2 datasets (left to right). The red line indicates the best performing baseline (SICL).}
\label{fig:practical_consideration}
\end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=.99\columnwidth]{pptx/adaptive-knn1_cropped.pdf}
% \includegraphics[width=.99\columnwidth]{pptx/adaptive-knn2_cropped.pdf}
% \caption{\textit{Left}: A sample test instance for which only a single example suffices for correct prediction.
% \textit{Right}: Another test instance for which only a single example does not result in the correct prediction. Increasing the number of examples results in the correct prediction (examples are shown in blue color).}
% \label{fig:icl-demo}
% \end{figure*}

==> figdefs/f1_vs_numDemo.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{figs/oracle_vs_similar.png}
\caption{
A comparison between in-context learning (ICL) with fixed number of examples ($k$) over a range from 0 to 5, and an oracle that chooses the smallest number of examples that leads to the highest probability for the correct class (experiments conducted on the AGNews text classification dataset). 
% If the downstream prediction is incorrect for all values of $k \in \{0,\ldots,5\}$, the oracle chooses the $0$-shot prediction. 
The comparison shows that using a variable number of examples performs better than static $k$-shot prompting, and motivates the research question on how to effectively predict the number of examples for a data instance (we intend to achieve results somewhere between the oracle and the static ICL).}
\label{fig:f1_vs_numDemo}
\end{figure}

==> figdefs/k_in_knn.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\columnwidth]{figs/k_in_knn.pdf}
% \caption{\small
% Binary classification using kNN with a fixed $k$ value, i.e., $k = 5$.}
% \label{fig:k_in_knn}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.75\columnwidth]{figs/apl_motivation_4_cropped.pdf}
\caption{
Motivation behind using a variable number of examples for ICL across the test instances: 1) The test sample `\textcolor{teal}{\textbf{?}}' is located within a homogeneous neighborhood of negative data points indicating that an LLM may perform well with only a few nearest neighbour demonstrations. 2) The test instance `\textcolor{darkgray}{\textbf{?}}' is located within a heterogeneous neighborhood, as a result of which, an LLM may require a higher number of such demonstrations to correctly predict its class. 
% 3) The test sample \textcolor{black}{\textbf{?}} is an outlier and even the nearest neighbours are fairly far away from it. In such cases, even $0$-shot prompts may perform better than few-shot because the not-so-similar neighbors may behave as noise for the LLM.
}
\label{fig:k_in_knn}
\end{figure}

==> figdefs/neighbourhood_ent.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.60\columnwidth]{figs/neighbourhood_ent_cropped.pdf}
\caption{
Influence of neighbourhood homogeneity on the smallest number of demonstrations that result in a correct prediction. 
}
\label{fig:neighbourhood_ent}
\end{figure}

==> figdefs/numdatapoints_vs_k.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.75\columnwidth]{figs/K_numdata_linepoint.pdf}
\caption{
Proportion of the smallest number of examples for each test instance in the SST2 \cite{sst2} dataset that lead to correct predictions.
%that results yields the highest probability for the correct class using ICL (results on the ; more details in Section \ref{sec:expsetup}).
}
\label{fig:numdatapoints_vs_k}
\end{figure}

==> figdefs/workflow.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.75\columnwidth]{figs/workflow_cropped.pdf}
    \caption{A diagram illustrating the workflow of Adaptive in-context learning (AICL). Section \ref{subsec:aicl} discusses possible ways of adapting the number of ICL examples.}
    \label{fig:workflow}
\end{figure}

==> sections/limitations.tex <==
\hlt{The main limitation of the proposed model is that it involves an additional computation step of learning the optimal number of examples to use. As is the case with supervised models, this requires certain amount of data for effectively learning this classification. Obtaining such a dataset involves invoking the LLM multiple times to find out the values of the number of examples that work. Our proposed approach makes use of the same LLM during training as well as inference time.}
% Our experiments reported in Figure \ref{fig:practical_consideration} suggests that the classifier to predict the optimal number of ICL examples does not work well with too few training samples (e.g., 10\% of the available training data).

Another limitation is that in our approach, the demonstrations are always sorted based on the semantic similarity with the test instance. However, the relative sequence of the demonstrations is not dynamically adapted.

% \hlt{Another limitation of the proposed methodology is that there is a performance gap between the oracle and AICL across dataset and LLM choices. This suggests that there is, indeed, scope for improvement to look for signals other than the topical content and the neighbourhood homogeneity to predict the number of appropriate ICL examples.}

% The possible reason behind this is that the input text alone may not be a clear discriminator for different values of $k$ and that some additional features may be required to be fed in.

% Furthermore, in our experiments, we use the same LLM for (a) performing predictions on the downstream task, and (b) constructing a dataset for training $\kappa$. For very large LLMs, it would be beneficial to use a smaller LLM for (b), since it involves running inferences on the train set (which is larger than the test set on which final predictions will be performed).

==> tabledefs/gpt-agnews.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-7}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
\midrule
0-shot & 0 & 0.6569 & 0.5932 & 0.5849 & 60 & 0.25 \\
RICL & 1 & 0.4585 & 0.4650 & 0.4522 & 123 & 0.31 \\
RICL & 3 & 0.6338 & 0.6189 & 0.5916 & 246 & 0.45 \\
RICL & 5 & 0.6746 & 0.6547 & 0.6354 & 370 & 0.58 \\
SICL & 1 & 0.9015 & 0.9017 & 0.9016 & 124 & 0.70 \\
SICL & 3 & 0.9006 & 0.8993 & 0.8985 & 252 & 0.86 \\
SICL & 5 & 0.8974 & 0.8938 & 0.8925 & 380 & 1.00 \\
AICL-L & 1.05 & 0.8725 & 0.8716 & 0.8709 & 128 & 0.71 \\
AICL-U & 1.87 & \textbf{0.9080} & \textbf{0.9096} & \textbf{0.9067} & 175 & 0.79 \\
\shade Oracle & \shade 1.08 &\shade 0.9521 &\shade 0.9518 &\shade 0.9517 &\shade 130 &\shade 0.71 \\
\bottomrule
\end{tabular}

==> tabledefs/gpt-ss2.tex <==
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
% \multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
% \cmidrule(r){1-2} \cmidrule(l){3-7}
% Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
% \midrule
% 0-shot & 0 & 0.7503 & 0.5022 & 0.3379 & 30 & 0.54 \\
% RICL & 1 & 0.8277 & 0.8258 & 0.8256 & 61 & 0.59 \\
% RICL & 3 & 0.9181 & 0.9159 & 0.9158 & 124 & 0.74 \\
% RICL & 5 & 0.9278 & 0.9269 & 0.9269 & 187 & 0.91 \\
% SICL & 1 & 0.8420 & 0.8412 & 0.8411 & 60 & 0.69 \\
% SICL & 3 & 0.9151 & 0.9148 & 0.9148 & 120 & 0.84 \\
% SICL & 5 & 0.9261 & 0.9253 & 0.9252 & 180 & 1.00 \\
% AICL-L & 1.09 & 0.8907 & 0.8885 & 0.8883 & 64 & 0.70 \\
% AICL-U & 4.12 & \textbf{0.9302} & \textbf{0.9304} & \textbf{0.9302} & 154 & 0.90 \\
% \shade Oracle & \shade 1.18 &\shade  0.9792 &\shade  0.9791 &\shade  0.9791 &\shade  66 &\shade  0.71 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{3}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\
\midrule
0-shot & 0 & 0.7532 & 0.5143 & 0.3639 \\
SICL & 1 & 0.6278 & 0.6077 & 0.5914 \\
SICL & 5 & 0.8054 & 0.7313 & 0.7137 \\
SICL & 10 & 0.8382 & 0.7840 & 0.7747 \\ \midrule
AICL(e) & 7.57 & 0.8322 & 0.7770 & 0.7671 \\
AICL(e+n) & 4.97 & \textbf{0.8506} & \textbf{0.8365} & \textbf{0.8347} \\
\shade Oracle & \shade 1.20 &\shade  0.9582 &\shade  0.9545 &\shade  0.9543 \\
\bottomrule
\end{tabular}

==> tabledefs/gpt-tox.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-7}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
\midrule
0-shot & 0 & 0.5689 & 0.6238 & 0.5769 & 103 & 0.22 \\
RICL & 1 & 0.5222 & 0.5573 & 0.4837 & 206 & 0.31 \\
RICL & 3 & 0.5221 & 0.5485 & 0.5153 & 410 & 0.48 \\
RICL & 5 & 0.5272 & 0.5642 & 0.5052 & 610 & 0.65 \\
SICL & 1 & 0.5751 & 0.6967 & 0.5490 & 203 & 0.69 \\
SICL & 3 & 0.6169 & 0.7223 & 0.6367 & 391 & 0.85 \\
SICL & 5 & 0.6078 & \textbf{0.7248} & 0.6217 & 431 & 1.00 \\
AICL-L & 1.26 & 0.6020 & 0.7159 & 0.6134 & 227 & 0.75 \\
AICL-U & 3.46 & \textbf{0.6197} & 0.7237 & \textbf{0.6401} & 359 & 0.90 \\
\shade Oracle & \shade 1.32 & \shade 0.7939 & \shade 0.8715 & \shade 0.8263 & \shade 231 & \shade 0.76 \\
\bottomrule
\end{tabular}

==> tabledefs/gpt-trec.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{3}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\
\midrule
0-shot & 0 &  &  &  \\
SICL & 1 &  &  &  \\
SICL & 5 &  &  &  \\
SICL & 10 &  &  &  \\ \midrule
AICL(e) &  &  &  &  \\
AICL(e+n) &  & \textbf{} & \textbf{} & \textbf{} \\
\shade Oracle & \shade  &\shade   &\shade   &\shade   \\
\bottomrule
\end{tabular}

==> tabledefs/llama-trec.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{3}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\
\midrule
0-shot & 0 & 0.4496 & 0.4088 & 0.1882 \\
SICL & 1 & 0.6135 & 0.6404 & 0.5548 \\
SICL & 5 & 0.7455 & 0.8321 & 0.7405 \\
SICL & 10 & 0.7457 & 0.7587 & 0.6880 \\ \midrule
AICL(e) & 9.42 & 0.8376 & 0.8736 & 0.8446 \\
AICL(e+n) & 9.44 & \textbf{0.8376} & \textbf{0.8770} & \textbf{0.8483} \\
\shade Oracle & \shade 1.78 &\shade  0.9225 &\shade  0.9719 &\shade  0.9422 \\
\bottomrule
\end{tabular}

==> tabledefs/opt-agnews.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-7}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
\midrule
0-shot & 0 & 0.7326 & 0.7222 & 0.7103 & 60 & 0.16 \\
RICL & 1 & 0.4154 & 0.4211 & 0.4145 & 123 & 0.25 \\
RICL & 3 & 0.6023 & 0.6028 & 0.5982 & 246 & 0.42 \\
RICL & 5 & 0.6548 & 0.6401 & 0.6395 & 370 & 0.61 \\
SICL & 1 & 0.9016 & 0.9017 & 0.9016 & 124 & 0.62 \\
SICL & 3 & 0.9058 & 0.9046 & 0.9044 & 252 & 0.80 \\
SICL & 5 & 0.8994 & 0.8945 & 0.8941 & 380 & 1.00 \\
AICL-L & 1.06 & 0.8907 & 0.8885 & 0.8883 & 129 & 0.64 \\
AICL-U & 1.91 & \textbf{0.9109} & \textbf{0.9088} & \textbf{0.9097} & 178 & 0.71 \\ 
\shade Oracle & \shade 1.08 & \shade 0.9470 & \shade 0.9467 & \shade 0.9467 & \shade 130 & \shade 0.65 \\
\bottomrule
\end{tabular}

==> tabledefs/opt-sst.tex <==
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
% \multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
% \cmidrule(r){1-2} \cmidrule(l){3-7}
% Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
% \midrule
% 0-shot & 0 & 0.7541 & 0.5170 & 0.3698 & 30 & 0.32 \\
% RICL & 1 & 0.8601 & 0.8260 & 0.8216 & 61 & 0.44 \\
% RICL & 3 & 0.8465 & 0.8314 & 0.8295 & 124 & 0.68 \\
% RICL & 5 & 0.8988 & 0.8886 & 0.8877 & 187 & 0.91 \\
% SICL & 1 & 0.8495 & 0.8150 & 0.8102 & 60 & 0.56 \\
% SICL & 3 & 0.8413 & 0.8270 & 0.8251 & 120 & 0.78 \\
% SICL & 5 & 0.8947 & 0.8885 & 0.8880 & 180 & 1.00 \\
% AICL-L & 1.11 & 0.8700 & 0.8600 & 0.8589 & 65 & 0.59 \\
% AICL-U & 4.93 & \textbf{0.9061} & \textbf{0.9013} & \textbf{0.9012} & 178 & 0.98 \\
% \shade Oracle & \shade 1.22 & \shade 0.9635 & \shade 0.9616 & \shade 0.9615 & \shade 67 & \shade 0.60 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{3}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-5}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ \\
\midrule
0-shot & 0 & 0.7722 & 0.6181 & 0.5547 \\
SICL & 1 & 0.5007 & 0.5007 & 0.4995 \\
SICL & 5 & 0.8386 & 0.8077 & 0.8030 \\
SICL & 10 & 0.8748 & 0.8707 & 0.8703 \\ \midrule
AICL(e) & 8.56 & 0.9118 & 0.8979 & 0.8968 \\
AICL(e+n) & 8.82 & \textbf{0.9150} & \textbf{0.9018} & \textbf{0.9009} \\
\shade Oracle & \shade 1.27 &\shade  0.9764 &\shade  0.9753 &\shade  0.9753 \\
\bottomrule
\end{tabular}

==> tabledefs/opt-tox.tex <==
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{5}{c}{Evaluation} \\
\cmidrule(r){1-2} \cmidrule(l){3-7}
Method & $k$ & Precision$\uparrow$ & Recall$\uparrow$ & F-score$\uparrow$ & AIS$\downarrow$ & RRT$\downarrow$ \\
\midrule
0-shot & 0 & 0.5498 & 0.5767 & 0.5553 & 103 & 0.17 \\
RICL & 1 & 0.5193 & 0.5424 & 0.5022 & 199 & 0.28 \\
RICL & 3 & 0.5250 & 0.5529 & 0.5129 & 367 & 0.50 \\
RICL & 5 & 0.5262 & 0.5562 & 0.5132 & 488 & 0.72 \\
SICL & 1 & 0.5860 & \textbf{0.6938} & 0.5876 & 195 & 0.75 \\
SICL & 3 & 0.5961 & 0.6889 & 0.6091 & 335 & 0.88 \\
SICL & 5 & 0.6023 & 0.6915 & 0.6184 & 431 & 1.00 \\
AICL-L & 1.24 & 0.5983 & 0.6881 & 0.6128 & 223 & 0.79 \\
AICL-U & 4.12 & \textbf{0.6164} & 0.6693 & \textbf{0.6223} & 398 & 0.93 \\ 
\shade Oracle & \shade 1.32 & \shade 0.7939 & \shade 0.8715 & \shade 0.8263 & \shade 231 & \shade 0.80 \\
\bottomrule
\end{tabular}

==> tabledefs/results.tex <==
\begin{table*}
\centering
\caption{A comparison of our proposed Adaptive ICL vs. the baselines on three datasets.
$k$: \#few-shot examples for baselines. For AICL, this denotes the average number of examples used.
\label{table:results}
}
\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular}{ll|llll|llll|llll|llll}
\toprule
\multicolumn{2}{c}{Settings} & \multicolumn{4}{c}{SST2} & \multicolumn{4}{c}{TREC} & \multicolumn{4}{c}{CoLA} & \multicolumn{4}{c}{RTE} \\
\cmidrule(r){1-2} \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14} \cmidrule(l){15-18}
Model & Method & $k$ & Precision & Recall & F-score & $k$ & Precision & Recall & F-score & $k$ & Precision & Recall & F-score & $k$ & Precision & Recall & F-score \\
\midrule
\multirow{5}{*}{Llama-2-7b} & 0-shot & 0 & 0.7585 & 0.6166 & 0.5564 & 0 & 0.1623 & 0.0200 & 0.0046 & 0 & 0.5905 & 0.6851 & 0.5719 & 0 & 0.4836 & 0.5199 & 0.3999  \\
 & FICL & 10 & 0.8828 & 0.8771 & 0.8767 & 8 & \textbf{0.8615} & 0.7380 & 0.7584 & 9 & 0.6830 & 0.6851 & 0.6789 & 8 & 0.6357 & 0.6209 & 0.6169 \\
 & AICL(E) & 8.61 & 0.9136 & 0.8995 & 0.8987 & 7.07 & 0.8453 & 0.8260 & 0.8271 & 5.34 & 0.6853 & 0.7106 & 0.6850 & 3.35 & 0.6529 & 0.6399 & 0.6378  \\
 & AICL(E+N) & 8.41 & \textbf{0.9161} & \textbf{0.9035} & \textbf{0.9028$^*$} & 6.64 & 0.8465 & \textbf{0.8340} & \textbf{0.8352$^*$} & 5.32 & \textbf{0.6982} & \textbf{0.7213} & \textbf{0.6933$^*$} & 4.02 & \textbf{0.6533} & \textbf{0.6411} & \textbf{0.6380$^*$} \\
 & \shade Oracle & \shade 1.27 & \shade 0.9765 & \shade 0.9753 & \shade 0.9753 & \shade 3.29  & \shade 0.9408  & \shade 0.9040 & \shade 0.9138 & \shade 0.53 & \shade 0.9887 & \shade 0.9885 & \shade 0.9884 & \shade 0.92 & \shade 0.9715 & \shade 0.9711 & \shade 0.9711 \\ \cmidrule{1-18}
 \multirow{5}{*}{Phi-2} & 0-shot & 0 & 0.8989 & 0.8918 & 0.8913 & 0 & 0.6285 & 0.3700 & 0.3097 & 0 & 0.4802 & 0.3126 & 0.1772 & 0 & 0.6751 & 0.6751 & 0.6751 \\
 & FICL & 10 & 0.9278 & 0.9253 & 0.9252 & 9 & 0.7972 & 0.6800 & 0.6871 & 2 & 0.7395 & \textbf{0.7526} & 0.7316 & 2 & 0.7333 & 0.7292 & 0.7261 \\
 & AICL(E) & 8.67 & 0.9351 & 0.9330 & 0.9329 & 4.62 & 0.8442 & 0.8290 & 0.8312 & 6.88 & 0.7501 & 0.7515 & 0.7457 & 4.83 & 0.7389 & 0.7451 & 0.7398 \\
 & AICL(E+N) & 5.09 & \textbf{0.9381} & \textbf{0.9374} & \textbf{0.9374$^*$} & 4.48 & \textbf{0.8486} & \textbf{0.8350} & \textbf{0.8362$^*$} & 5.93 & \textbf{0.7588} & 0.7518 & \textbf{0.7491$^*$} & 5.10 & \textbf{0.7467} & \textbf{0.7418} & \textbf{0.7405$^*$} \\
 & \shade Oracle & \shade 0.18 & \shade 0.9870 & \shade 0.9868 & \shade 0.9868 & \shade 1.30 & \shade 0.9649 & \shade 0.9640 & \shade 0.9642 & \shade 0.57 & \shade 0.9786 & \shade 0.9779 & \shade 0.9777 & \shade 0.83 & \shade 0.9307 & \shade 0.9278 & \shade 0.9275  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

==> tabledefs/results_newfmt.tex <==
\begin{table*}[t]
\centering
\caption{
A comparison of our proposed adaptive ICL vs. the baselines on \sth{several} \hlt{two} datasets.
$k$: \#few-shot examples for baselines. For AICL, this denotes the average number of examples used. AIS: average input size (\#tokens) rounded off to the nearest integer. \sth{RRT: run-time relative to $5$-shot (lower the RRT, the faster is the inference)}.
%of the respective method relative to that of SICL with $k=5$.
\label{table:results}
}
%
% \begin{subtable}{.95\columnwidth} % change this for smaller tables
% \begin{adjustbox}{width=.99\columnwidth} % don't change these
% \input{tabledefs/opt-agnews}
% \end{adjustbox}
% \caption{LLaMA-2-7B on AGNews \label{tab:agnews_opt}}
% \end{subtable}
% \quad
% %
% \begin{subtable}{.95\columnwidth}
% \begin{adjustbox}{width=.99\columnwidth}
% \input{tabledefs/gpt-agnews}
% \end{adjustbox}
% \caption{GPT-J on AGNews \label{tab:agnews_gpt}}
% \end{subtable}
%
% \begin{subtable}{.95\columnwidth}
% \begin{adjustbox}{width=.99\columnwidth}
% \input{tabledefs/opt-tox}
% \end{adjustbox}
% \caption{OPT-2.7B on Toxicity \label{tab:agnews_opt}}
% \end{subtable}
% \quad
% %
% \begin{subtable}{.95\columnwidth}
% \begin{adjustbox}{width=.99\columnwidth}
% \input{tabledefs/gpt-tox}
% \end{adjustbox}
% \caption{GPT-J on Toxicity \label{tab:agnews_gpt}}
% \end{subtable}
%
\begin{subtable}{.95\columnwidth}
\begin{adjustbox}{width=.95\columnwidth}
\input{tabledefs/opt-sst}
\end{adjustbox}
\caption{LLAMA-2-7B on SST2 \label{tab:agnews_opt}}
\end{subtable}
\quad
%
\begin{subtable}{.95\columnwidth}
\begin{adjustbox}{width=.95\columnwidth}
\input{tabledefs/gpt-ss2}
\end{adjustbox}
\caption{GPT-J on SST2 \label{tab:agnews_gpt}}
\end{subtable}
% 
\begin{subtable}{.95\columnwidth}
\begin{adjustbox}{width=.95\columnwidth}
\input{tabledefs/llama-trec}
\end{adjustbox}
\caption{LLAMA-2-7B on TREC \label{tab:agnews_opt}}
\end{subtable}
\quad
%
\begin{subtable}{.95\columnwidth}
\begin{adjustbox}{width=.95\columnwidth}
\input{tabledefs/gpt-trec}
\end{adjustbox}
\caption{GPT-J on TREC \label{tab:agnews_gpt}}
\end{subtable}
\end{table*}
